NISQ+: Boosting quantum computing power by approximating quantum error correction

Quantum computers are growing in size, and design decisions are being made now that attempt to squeeze more computation out of these machines. In this spirit, we design a method to boost the computational power of near-term quantum computers by adapting protocols used in quantum error correction to implement "Approximate Quantum Error Correction (AQEC)." By approximating fully-fledged error correction mechanisms, we can increase the compute volume (qubits $\times$ gates, or "Simple Quantum Volume (SQV)") of near-term machines. The crux of our design is a fast hardware decoder that can approximately decode detected error syndromes rapidly. Specifically, we demonstrate a proof-of-concept that approximate error decoding can be accomplished online in near-term quantum systems by designing and implementing a novel algorithm in Single-Flux Quantum (SFQ) superconducting logic technology. This avoids a critical decoding backlog, hidden in all offline decoding schemes, that leads to idle time exponential in the number of T gates in a program. Our design utilizes one SFQ processing module per physical qubit. Employing state-of-the-art SFQ synthesis tools, we show that the circuit area, power, and latency are within the constraints of contemporary quantum system designs. Under pure dephasing error models, the proposed accelerator and AQEC solution is able to expand SQV by factors between 3,402 and 11,163 on expected near-term machines. The decoder achieves a $5\%$ accuracy-threshold and pseudo-thresholds of $\sim$ $5\%, 4.75\%, 4.5\%,$ and $3.5\%$ physical error-rates for code distances $3, 5, 7,$ and $9$. Decoding solutions are achieved in a maximum of $\sim 20$ nanoseconds on the largest code distances studied. By avoiding the exponential idle time in offline decoders, we achieve a $10$x reduction in required code distances to achieve the same logical performance as alternative designs.

==> approach.tex <==
\section{Our Approach}\label{sec:approach}
\subsection{High level description of design}
We introduce an accelerator layer designed in SFQ logic, that is placed on top of our quantum bits. The ancilla qubits measure the syndromes by interacting with data qubits, and then send the measurement results to the accelerator layer. The accelerator is then responsible for finding the chains of errors that connect syndrome changes. Chains of errors are then sent to a higher level classical controller in order to correct the errors.

The accelerator layer is built in a two dimensional array of the hardware blocks called \emph{Accelerator Block}. There is one \emph{Accelerator Block} per each ancilla qubit. Each \emph{Accelerator Block} has five inputs; one input that comes from the corresponding ancilla qubit that shows the syndrome change, and four other inputs that comes from the adjacent \emph{Accelerator Blocks}. Each \emph{Accelerator Block} also has five outputs. Four outputs that goes to the adjacent \emph{Accelerator Blocks}, and one other output called \emph{chain} output that tells the higher level classical computer that the \emph{Accelerator Blocks} is part of the chain. Chain calculation in the accelerator layer proceeds by sequentially growing a search space around each hot syndrome. 

\iffalse
\begin{itemize}
    \item Architecture: In high level, how does the system work?
    \item Chains are calculated and sent to classical computers in order to correct the errors.
    \item Chain calculation proceeds by sequentially growing a search space around each hot syndrome until parity within each syndrome region becomes even.
    \item At this point pairs of syndromes and the corresponding paths between them are returned to a higher level classical controller.
\end{itemize}
\fi
  
\subsection{Detailed description of design}
\subsubsection{Circuit Description}
Each \emph{Accelerator Block} with syndrome change propagate a signal to four directions; in first cycle, it sends the signal to all the adjacent \emph{Accelerator Blocks}, and then the signal propagates sequentially in each direction. We need a flip-flop at each \emph{Accelerator Block} to determine whether or not it is part of the propagation process. The propagation process continues until an \emph{Accelerator Block} called \emph{Joint Accelerator Block} receives signals from two different directions meaning two different \emph{Accelerator Block} with syndrome change are propagating signals at the same time; then, the \emph{Joint Accelerator Block} send output signals to directions that it received the signals from. The \emph{Accelerator Blocks} that were part of the propagation process and now receives signal from the \emph{Joint Accelerator Block} turn on their \emph{chain} output, and sends the signal to the next \emph{Accelerator Blocks}. Thus, the \emph{chain} output of a chain of \emph{Accelerator Blocks} is turned on in one cycle. Finally, we need the \emph{chain} outputs to be turned off at the next cycle (as the classical controller already received them), thus, we connect the \emph{chain} output to the reset port of the flip-flops.

\subsubsection{Circuit Simulation}
We drew a schematic of our circuits and converted the design to verilog code using Logisim \cite{logisim}. We used V2C \cite{v2c} to convert the verilog code to the C code. We then connect the C code to an in-house simulator to simulate the effectiveness of our design. Our in-house simulator generates errors and feed them to our design, and then collect the calculated chains and compare them with an ideal QEC system, and finally calculates the accuracy of our design in detecting the errors.

\subsubsection{Circuit Synthesize}
We synthesized our SFQ circuits using the process explained in \cite{synthesise}

\iffalse
\begin{itemize}
  \item Circuit: Detail of the SFQ circuits we designed. 
  \item Device: Detail of the SFQ logic and cell library we used. 
  \item Tools we used to synthesize the circuits.
  \item Tools we used to simulate the circuits. 
\end{itemize}
\fi

==> circuitdesign.tex <==
\section{Circuit Design Considerations}\label{sec:circuitdesign}

In this section we explicitly and formally describe the decoding algorithm that we have designed, as well as circuit design rules upon which we construct the \emph{Accelerator Blocks}. Below is the summary of all the circuit design considerations that we have.
 
\begin{figure}[!ht]
  \begin{center}
  \includegraphics[width=0.7\linewidth]{circuitrule.pdf}
  \caption{Scenarios where a syndrom change can be a part of multiple error chains, and we need to break the tie.}
  \label{circuitrule}
  \end{center}
\end{figure}
 
 
\begin{enumerate}
    \item We need to find error chains that connect syndrome changes, as well as the error chains that connect syndrome changes to boundaries of the quantum grid. Note that we need to prioritize the error chains that connect the syndrome changes as they have higher probability of happening. Thus, we need to have a way to differentiate the two different type of error chains and in the case they both happen at the same time, choose the one with higher probability.
    \item When a syndrome change is part of more than one error chain at the same cycle, and all the chains has equal probability of happening, we need to break the tie. Examples of such scenario are 1) when a syndrome change is matched with more than one boundary, 2) when one syndrome change has equal distance to different syndrome change as shown in Figure \ref{circuitrule}.
    \item We need to stop the growth of syndrome changes after they are matched with another syndrome change or a boundary. We assume there is a signal coming from the classical control that disable the syndrome change.
    \item We also need to reset the flip-flops that are set in the phase that syndrome change was growing, after the syndrome change is matched.
\end{enumerate}

==> future.tex <==
There are a number of immediate extensions to this work:

\begin{itemize}
    \item \emph{Circuit Optimizations}
    \item \emph{Magic State Distillation Acceleration}
\end{itemize}

==> quantumerrorcorrection.tex <==
\subsection{What is Quantum Error Correction?}
\subsection{Stabilizer Codes}
\subsection{Topological Code Decoding}

==> results.tex <==
\section{Results}\label{sec:results}
Our results show that we have similar accuracy than Blossom algorithm (that is based on minimum-weight perfect matching \cite{blossom}), as we both can achieve 5-6\% accuracy threshold when we do not consider matching with the boundaries. By adding the boundary matching to the algorithm the accuracy threshold of Blossom algorithm increases 10.3\%. We are in the process of adding the boundary matching to our circuits as well, and we expect to provide the same accuracy threshold. Note that the accuracy threshold is the threshold of injecting physical errors so that the logical error decreases by increasing the grid size.

We are able to achieve the same accuracy threshold than the previously proposed QEC techniques, while providing higher speed. Considering 800ns as the time required to do one round of syndrome measurements and 50Ghz as the frequency of the SFQ logic, we can have 40,000 cycles to match all the syndrome changes. Thus, even considering large syndrome grids of size 20,000 x 20,000, we are still able to match all the syndrome changes in 800ns (note that the maximum time requires to match two syndrome is 40,000 in a 20,000 x 20,000 grid and it happens when the top-left syndrome change wants to match with the bottom-right syndrome change).


%\begin{itemize}
%  \item Accuracy vs speed trade-off in our approach compared to previous work.
%  \item Sensitivity on grid size and error rate
%  \item Discussion about power/latency/area characteristics of each design
%  \item Sweep across different design iterations that capture more accuracy at the expense of physical footprint
%\end{itemize}

==> scheduling.tex <==
\section{Scheduling}\label{sec:scheduling}



This section describes the impact of instruction level optimizations: gate scheduling and qubit reuse. A \emph{schedule} of a quantum program is a sequence of gate operations on logical qubits. The sequence ordering defines \emph{data dependencies} between gates, where a gate $g_1$ depends on $g_0$ if they share a logical qubit and $g_1$ appears later in the schedule sequence than $g_0$.

\subsection{Gate Scheduling}
The impact of gate scheduling can be quite significant in quantum circuits, and many algorithm implementations rely upon the execution of gates in parallel in order to achieve substantial algorithmic speedup. Gate scheduling in quantum algorithms differs from classical instruction scheduling, as gate commutativity introduces another degree of freedom for schedulers to consider. Compared to the field of classical instruction scheduling, quantum gate scheduling has been relatively understudied, with only few systematic approaches being proposed that incorporate these new constraints \cite{gianScheduling}. 

In exploring these effects applied to Bravyi-Haah state distillation circuits, we find that these optimizations are limited in their effectiveness. While intuitively the modularity of the block code construction would allow for early execution of gates arising in late rounds of the distillation procedure, the \textit{checkpoints} required to implement module checking as described in section \ref{subsec:block} limit the magnitude of gate mobility.

The structure of the block code circuitry only allows for a small constant number of gates to by executed early, outside of the rounds from which they originate. Because of this, the maximum critical path extension by the introduction of a \emph{barrier} preventing gate mobility outside of the originating round is equal to this small constant multiplied by the number of block code iterations. The benefit of inserting a barrier at the end of each round is to create clean divisions between the rounds. As Fig.~\ref{fig:interactiongraphs} shows, the interaction graph for a single round is a planar graph, while this planarity is destroyed as rounds are added. Barriers expose this planarity, making the circuit easier to map. Barriers in these circuits can be inserted by adding a multi-target CNOT operation into the schedule, controlled by an ancilla qubit initialized into a logical $\ket{0}$ state, and targeting all of the qubits that the schedule wishes to constrain.

Additionally, gate scheduling order has significant impacts on network congestion. Scheduling these small constant number of gates early therefore runs the risk of causing congestion with previous round activity. This can in fact extend the circuit latency, even though the circuit has executed gates earlier in the schedule. 

Overall, the insertion of a barrier appears to not significantly alter the schedule of circuit gates. It does, however, change the interaction between the schedule and a particular physical qubit mapping. This relationship will be explored in more detail in Section \ref{sec:optimize}.




\subsection{Qubit Reuse}
We show in this section that an important schedule characteristic of the block protocol to leverage is the hierarchical structure of the distillation circuit. Between two rounds of the procedure, all ancillary qubits will be measured for error checking at the end of the previous round, and reinitialized at the beginning of the next round. This type of data qubit sharing (which we call ``sharing-after-measurement'') is a \emph{false dependency}, because they can be resolved by qubit renaming. Now this naturally leads to the question: (how) should we reuse the qubits between multiple rounds? 

The first approach we explore is to prevent any false sharing of the qubits, at the cost of larger area, by always allocating new data qubits for different rounds. This removes all dependencies due to ancillary qubits, leaving only true dependencies on qubits generated in the previous round. This minimizes execution time at the cost of extra qubits (and space). 

The second approach is to strategically choose which qubits from the previous round to be reused for the next. This approach directly reduces the area needed for the entire factory, at the cost of introducing false dependencies. 

In order to make intelligent decisions on which set of ancillary qubits to reuse, it requires us to have information about the topological mapping of the qubits, since mapping and reuse decisions together significantly influence the congestion overhead of the circuit. We will discuss the subtleties of the tradeoff in more detail later in Section \ref{sec:optimize}.


